The Geometry of the Painlev\'e paradox

Painlev\'e showed that there can be inconsistency and indeterminacy in solutions to the equations of motion of a 2D rigid body moving on a sufficiently rough surface. The study of Painlev\'e paradoxes in 3D has received far less attention. In this paper, we highlight the pivotal role in the dynamics of the azimuthal angular velocity Psi by proving the existence of three critical values of Psi, one of which occurs independently of any paradox. We show that the 2D problem is highly singular and uncover a rich geometry in the 3D problem which we use to explain recent numerical results.

==> 3D Painleve (SIADS)/ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}

\usepackage{cite}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

\usepackage{xfrac}
\usepackage{animate}
\usepackage{enumerate}
\usepackage[shortlabels]{enumitem}
\usepackage[a4paper,margin=25mm]{geometry}    % page layout
\usepackage{setspace} \singlespacing        % line spacing
\usepackage{amsfonts,amssymb,amsmath}         % useful math extensions
\usepackage{graphicx}                         % graphics import
\usepackage{siunitx}                          % easy SI units
%\usepackage{natbib}							  % bibliography 
\usepackage{hyperref}						  % good for urls
\usepackage{subcaption}						  % for subfigures
\usepackage{wrapfig}						  % wrap around figures
\usepackage{lipsum} 
\usepackage{xcolor}
\definecolor{myblue}{rgb}{.1, .4, .8}
\definecolor{myred}{rgb}{.8, .1, .1}
\definecolor{myyellow}{RGB}{246,235, 24}
\definecolor{mylime}{RGB}{150,201, 61}
\definecolor{mypurple}{RGB}{186,83, 159}
\definecolor{myorange}{RGB}{246,134, 59}
\definecolor{matlab1}{rgb}{0, 0.4470, 0.7410}
\definecolor{matlab2}{rgb}{0.8500, 0.3250, 0.0980}
\definecolor{matlab3}{rgb}{0.9290, 0.6940, 0.1250}
\definecolor{matlab4}{rgb}{0.4940, 0.1840, 0.5560}
\usepackage[usestackEOL]{stackengine}
\usepackage[T1]{fontenc}
\usepackage{animate}
\usepackage{booktabs}
\usepackage{longtable}
\usepackage{adjustbox}
\usepackage{mdframed}
\usepackage{todonotes}
\usepackage{xargs}
\usepackage{xstring}



% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\crefname{remark}{Remark}{Remark}
\crefname{Example}{Example}{Examples}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}
\newsiamremark{assumption}{Assumption}
\crefname{assumption}{Assumption}{Assumption}

% Sets running headers as well as PDF title and authors
\headers{The Geometry of the Painlev\'e paradox}{ N. Cheesman, S. J. Hogan, K. Uldall Kristiansen}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{The Geometry of the Painlev\'e paradox\thanks{Submitted to the editors {26/10/2021}.
\funding{{This work was funded by the UK Engineering and Physical Sciences Research Council (EPSRC) as part of the first author's PhD Studentship.}}}}

% Authors: full names plus addresses.
\author{
Noah Cheesman\thanks{Department of Engineering Mathematics, University of Bristol, Bristol BS8 1TW, UK
(\email{noah.cheesman@bristol.ac.uk}, \email{s.j.hogan@bristol.ac.uk}).}
 \and S.J. Hogan\footnotemark[2]
\and Kristian Uldall Kristiansen\thanks{Department of Applied Mathematics and Computer Science, Technical University of Denmark, 2800 Kgs. Lyngby, Denmark  
  (\email{krkri@dtu.dk}).}}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 
% User-defined commands
\newcommand{\diff}[2]{\frac{\mathrm{d}{#1}}{\mathrm{d}{#2}}}				% first derivative
\newcommand{\ddiff}[2]{\frac{\mathrm{d}^2{#1}}{\mathrm{d}{#2}^2}}			% second derivative
\newcommand{\pdiff}[2]{\frac{\partial{#1}}{\partial{#2}}}					% first partial
\newcommand{\pddiff}[2]{\frac{\partial^2{#1}}{\partial{#2}^2}}				% second partial
\newcommand{\pdiffdiff}[3]{\frac{\partial^2{#1}}{\partial{#2}\partial{#3}}}	%partial 2
\renewcommand{\vec}[1]{\boldsymbol{#1}}										%vector
\newcommand{\Idx}{\;\mathrm{d}x}
\newcommand{\Real}{\mathbb{R}}
\newcommand{\Complex}{\mathbb{C}}
\newcommand{\Rational}{\mathbb{Q}}
\newcommand{\Integer}{\mathbb{Z}}
\newcommand{\Natural}{\mathbb{N}}
\newcommand{\sgn}{\mathrm{sgn}}
\newcommand{\pe}{\text{pseudo-equilibrium}\ }
\newcommand{\pes}{\text{pseudo-equilibria}\ }
\newcommand{\titlemath}[1]{\texorpdfstring{#1}{TEXT}}
\newcommand{\tm}[1]{\texorpdfstring{#1}{TEXT}}
\newcommand{\sign}{\mathrm{sign}}
\def\dunderline#1{\underline{\underline{#1}}}
\newcommand{\indiff}[2]{\mathrm{d}{#1}/\mathrm{d}{#2}}
\newcommand{\tr}{\mathrm{tr}}		
\newcommand{\tangspace}{{\mathcal{T}}_{\mathbf{x}_0}\Sigma}
\newcommand{\orthcomp}{{\mathcal{O}}_{\mathbf{x}_0}\Sigma}		
\renewcommand{\vec}[1]{{#1}}
\renewcommand{\vec}[1]{\mathbf{#1}}
\newcommand{\mat}[1]{\mathbf{#1}}
\renewcommand{\mat}[1]{\underline{\vec{#1}}}
\renewcommand{\mat}[1]{{\underline{\underline{\mathrm{\smash{#1}}}}}}
\renewcommand{\vec}[1]{\underline{\smash{#1}}}
\DeclareMathOperator{\arctantwo}{arctan2}




%\allowdisplaybreaks

\usepackage{overpic}
%\usepackage{cleveref}

\usepackage{multirow}

% mywidehat
\usepackage{scalerel}

\newcommand\wh[1]{\hstretch{2}{\hat{\hstretch{.5}{#1}}}}


\renewcommand\eminnershape{\bfseries}

% Commenting
\usepackage{todonotes}
\newcommandx{\john}[2][1=]{\todo[linecolor=red,backgroundcolor=red!25,bordercolor=red,#1]{#2}}
\newcommandx{\johnin}[2][1=]{\todo[inline,linecolor=red,backgroundcolor=red!25,bordercolor=red,#1]{#2}}
\newcommandx{\noah}[2][1=]{\todo[linecolor=blue,backgroundcolor=blue!25,bordercolor=blue,#1]{#2}}
\newcommandx{\noahin}[2][1=]{\todo[inline,linecolor=blue,backgroundcolor=blue!25,bordercolor=blue,#1]{#2}}
\newcommandx{\kristian}[2][1=]{\todo[linecolor=green,backgroundcolor=green!25,bordercolor=green,#1]{#2}}
\newcommandx{\kristianin}[2][1=]{\todo[inline,linecolor=green,backgroundcolor=green!25,bordercolor=green,#1]{#2}}




\newlist{thmlist}{enumerate*}{1}
\setlist[thmlist]{label=\rm{(\arabic*)}}   


\crefname{thmlisti}{thm}{thms}
\creflabelformat{thmlisti}{#2#1#3}




\newcommand{\greentick}{$\color[rgb]{0,0.5,0}{\checkmark}$}
\newcommand{\ugreentick}{$\underline{\color[rgb]{0,0.5,0}{\checkmark}}$}
\newcommand{\redcross}{$\color[rgb]{0.5,0,0}{\times}$}
\newcommand{\redccross}{$\color[rgb]{0.5,0,0}{\otimes}$}

\usepackage[normalem]{ulem}

\definecolor{myblue}{rgb}{.1, .4, .8}
\definecolor{myred}{rgb}{.8, .1, .1}
%\definecolor{myyellow}{RGB}{246,235, 24}
\definecolor{myyellow}{rgb}{0.9647,0.9216,0.0941}
%\definecolor{mylime}{RGB}{150,201, 61}
\definecolor{mylime}{rgb}{0.5882,0.7882,0.2392}
%\definecolor{mypurple}{RGB}{186,83, 159}
\definecolor{mypurple}{rgb}{0.7294,0.3255,0.6235}
%\definecolor{myorange}{RGB}{246,134, 59}
\definecolor{myorange}{rgb}{0.9647,0.5255,0.2314}
\definecolor{md1}{rgb}{0, 0.4470, 0.7410}
\definecolor{md2}{rgb}{0.8500, 0.3250, 0.0980}
\definecolor{md3}{rgb}{0.9290, 0.6940, 0.1250}
\definecolor{md4}{rgb}{0.4940, 0.1840, 0.5560}
\definecolor{md5}{rgb}{0.4660, 0.6740, 0.1880}
\definecolor{md6}{rgb}{0.3010, 0.7450, 0.9330}
\definecolor{md7}{rgb}{0.6350, 0.0780, 0.1840}
\usepackage{multirow}



\usepackage{amssymb}

\usepackage{tikz}
\usepackage{pgfplots}
\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
            \node[shape=circle,draw,inner sep=2pt] (char) {#1};}}


%\usepackage{circledsteps}
%\newcommand{\circled}[1]{\Circled{#1}}

\usepackage{xargs}


% txfonts
\DeclareSymbolFont{matha}{OML}{txmi}{m}{it}
\DeclareMathSymbol{\varv}{\mathord}{matha}{118}
\DeclareMathOperator{\Tr}{tr}
\usepackage{overpic}

%%%%% delete next line when finished - something to do with todo fitting the PRSA format
\setlength{\marginparwidth}{2cm}
\usepackage{todonotes}
%%%%%%%%%%%% to separate out our comments

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Not sure if this is incompatible with RSPA's figure style
\usepackage{subcaption}
%Using the RPSA Figure fonts - looks funny - comment out unless necessary 
%\def\captionfont{\fontfamily{\sfdefault}\fontseries{m}\fontshape{n}\fontsize{8.5}{10}\selectfont}
%\def\captionheadfont{\fontfamily{\sfdefault}\fontseries{b}\fontshape{n}\fontsize{8.5}{10}\selectfont\raggedright}
%trying to bridge the gap in aesthetics
\captionsetup[figure]{labelfont=bf,labelsep=period}
\captionsetup[subfigure]{labelfont=normalfont}

\renewcommand{\vec}[1]{\boldsymbol{\mathbf{#1}}}
\renewcommand{\mat}[1]{\underline{\vec{#1}}}	
\renewcommand{\diff}[2]{\frac{\mathrm{d}{#1}}{\mathrm{d}{#2}}}
\renewcommand{\pdiff}[2]{\frac{\partial{#1}}{\partial{#2}}}
\renewcommand{\sign}[1]{\mathrm{sign}{#1}}








%Using Siam cleverref as I couldn't find PRSA style guidlines for referencing
%% Adding cleveref package for smart citations, with customizations to
%% make it act like SIAM expects.
\RequirePackage[capitalize,nameinlink]{cleveref}[0.19]

% Per SIAM Style Manual, "section" should be lowercase
\crefname{section}{section}{sections}
\crefname{subsection}{subsection}{subsections}
\Crefname{section}{Section}{Sections}
\Crefname{subsection}{Subsection}{Subsections}

% Per SIAM Style Manual, "Figure" should be spelled out in references
\Crefname{figure}{Figure}{Figures}

% Per SIAM Style Manual, don't say equation in front on an equation.
\crefformat{equation}{\textup{#2(#1)#3}}
\crefrangeformat{equation}{\textup{#3(#1)#4--#5(#2)#6}}
\crefmultiformat{equation}{\textup{#2(#1)#3}}{ and \textup{#2(#1)#3}}
{, \textup{#2(#1)#3}}{, and \textup{#2(#1)#3}}
\crefrangemultiformat{equation}{\textup{#3(#1)#4--#5(#2)#6}}%
{ and \textup{#3(#1)#4--#5(#2)#6}}{, \textup{#3(#1)#4--#5(#2)#6}}{, and \textup{#3(#1)#4--#5(#2)#6}}

% But spell it out at the beginning of a sentence.
\Crefformat{equation}{#2Equation~\textup{(#1)}#3}
\Crefrangeformat{equation}{Equations~\textup{#3(#1)#4--#5(#2)#6}}
\Crefmultiformat{equation}{Equations~\textup{#2(#1)#3}}{ and \textup{#2(#1)#3}}
{, \textup{#2(#1)#3}}{, and \textup{#2(#1)#3}}
\Crefrangemultiformat{equation}{Equations~\textup{#3(#1)#4--#5(#2)#6}}%
{ and \textup{#3(#1)#4--#5(#2)#6}}{, \textup{#3(#1)#4--#5(#2)#6}}{, and \textup{#3(#1)#4--#5(#2)#6}}

% Make number non-italic in any environment.
\crefdefaultlabelformat{#2\textup{#1}#3}

%\labelformat{subsection}{\thesection#1}


%Make own enumerates
\usepackage[shortlabels]{enumitem} 



\newlist{mycases}{enumerate}{3}
\setlist[mycases,1]{label=\textbf{Case~\arabic*},
                   ref  =\arabic*}
\setlist[mycases,2]{label=\textbf{(\alph*)},
                   ref  =\themyenumi\textbf{(\alph*)}}
\setlist[mycases,3]{label=\bfseries(\roman*),
                   ref  =\themyenumii\textbf{.(\roman*)}}

\crefname{mycasesi}{Case}{Cases}
\crefname{mycasesii}{item}{items}
\crefname{mycasesiii}{item}{items}


\newlist{mymechs}{enumerate}{3}
\setlist[mymechs,1]{label=\textbullet,
                   ref  =\Roman*}
\setlist[mymechs,2]{label=--,
                   ref  =\themymechsi\textbf{(\alph*)}}
\setlist[mymechs,3]{label=\bfseries(\roman*),
                   ref  =\themymechsii\textbf{.(\roman*)}}

\crefname{mymechsi}{Mechanism}{Mechanisms}
\crefname{mymechsii}{item}{items}
\crefname{mymechsiii}{item}{items}
\pgfplotsset{compat=1.16}
